Learning to Grasp the Ungraspable with Emergent Extrinsic Dexterity

A simple gripper can solve more complex manipulation tasks if it can utilize the external environment such as pushing the object against the table or a vertical wall, known as "Extrinsic Dexterity." Previous work in extrinsic dexterity usually has careful assumptions about contacts which impose restrictions on robot design, robot motions, and the variations of the physical parameters. In this work, we develop a system based on reinforcement learning (RL) to address these limitations. We study the task of "Occluded Grasping" which aims to grasp the object in configurations that are initially occluded; the robot needs to move the object into a configuration from which these grasps can be achieved. We present a system with model-free RL that successfully achieves this task using a simple gripper with extrinsic dexterity. The policy learns emergent behaviors of pushing the object against the wall to rotate and then grasp it without additional reward terms on extrinsic dexterity. We discuss important components of the system including the design of the RL problem, multi-grasp training and selection, and policy generalization with automatic curriculum. Most importantly, the policy trained in simulation is zero-shot transferred to a physical robot. It demonstrates dynamic and contact-rich motions with a simple gripper that generalizes across objects with various size, density, surface friction, and shape with a 78% success rate. Videos can be found at https://sites.google.com/view/grasp-ungraspable/.

==> table-success.tex <==
\begin{table}[H]
\caption{Each strategy being used in the successful episodes during real robot evaluation for \textbf{Policy w/ ADR}. A single policy network may execute either the dropping or standing strategy.}
\label{tab:success-1}
\vspace{3mm}
\centering

\scalebox{0.9}{
\begin{tabular}{lcc}
\hline
\textbf{} & \multicolumn{1}{l}{\textbf{Dropping}} & \multicolumn{1}{l}{\textbf{Standing}} \\ \hline
\textbf{Box-0} & 5 & 4 \\
\textbf{Box-0 + 4 erasers} & 8 & 2 \\
\textbf{Box-0 + 8 erasers} & 4 & 0 \\
\textbf{Box-1} & 1 & 7 \\
\textbf{Box-2} & 1 & 8 \\
\textbf{Box-3} & 5 & 3 \\
\textbf{Toy Bag} & 7 & 0 \\
\textbf{Bottle} & 1 & 7 \\
\textbf{Container} & 0 & 10 \\
\textbf{Container-reverse} & 0 & 6 \\ \hline
\textbf{Total} & \textbf{32} & \textbf{47} \\
\textbf{Percentage} & \textbf{40.5\%} & \textbf{59.5\%} \\ \hline
\end{tabular}}
\end{table}

        
% \begin{table}[H]
% \centering
%     \begin{minipage}{.48\linewidth}
%         \caption{Each strategy being used in the successful episodes during real robot evaluation for \textbf{Policy w/ ADR}. A single policy network may execute either the dropping or standing strategy.}
%         \label{tab:success-1}
%         \vspace{3mm}
%         \centering
        
%         \scalebox{0.9}{
%         \begin{tabular}{lrr}
%         \hline
%         \textbf{} & \multicolumn{1}{l}{\textbf{Dropping}} & \multicolumn{1}{l}{\textbf{Standing}} \\ \hline
%         \textbf{Box-0} & 5 & 4 \\
%         \textbf{Box-0 + 4 erasers} & 8 & 2 \\
%         \textbf{Box-0 + 8 erasers} & 4 & 0 \\
%         \textbf{Box-1} & 1 & 7 \\
%         \textbf{Box-2} & 1 & 8 \\
%         \textbf{Box-3} & 5 & 3 \\
%         \textbf{Toy Bag} & 7 & 0 \\
%         \textbf{Bottle} & 1 & 7 \\
%         \textbf{Container} & 0 & 10 \\
%         \textbf{Container-reverse} & 0 & 6 \\ \hline
%         \textbf{Total} & \textbf{32} & \textbf{47} \\ \hline
%         \end{tabular}}
%     \end{minipage}
%     \hspace{2mm}
%     \begin{minipage}{.48\linewidth}
%         \caption{Each strategy being used in the successful episodes during real robot evaluation for \textbf{Policy w/o ADR}. This policy tends to use the standing policy more often.}
%         \label{tab:success-2}
%         \vspace{3mm}
%         \centering
        
%         \scalebox{0.9}{
%         \begin{tabular}{lrr}
%         \hline
%         \textbf{} & \multicolumn{1}{l}{\textbf{Dropping}} & \multicolumn{1}{l}{\textbf{Standing}} \\ \hline
%         \textbf{Box-0} & 0 & 9 \\
%         \textbf{Box-0 + 4 erasers} & 0 & 6 \\
%         \textbf{Box-0 + 8 erasers} & 2 & 1 \\
%         \textbf{Box-1} & 0 & 5 \\
%         \textbf{Box-2} & 0 & 2 \\
%         \textbf{Box-3} & 0 & 0 \\
%         \textbf{Toy Bag} & 1 & 6 \\
%         \textbf{Bottle} & 0 & 0 \\
%         \textbf{Container} & 0 & 0 \\
%         \textbf{Container-reverse} & 0 & 0 \\ \hline
%         \textbf{Total} & \textbf{3} & \textbf{29} \\ \hline
%         \end{tabular}}
%     \end{minipage}
% \end{table}


